Hierarchical Adaptive Structural SVM for Domain Adaptation

A key topic in classification is the accuracy loss produced when the data distribution in the training (source) domain differs from that in the testing (target) domain. This is being recognized as a very relevant problem for many computer vision tasks such as image classification, object detection, and object category recognition. In this paper, we present a novel domain adaptation method that leverages multiple target domains (or sub-domains) in a hierarchical adaptation tree. The core idea is to exploit the commonalities and differences of the jointly considered target domains. Given the relevance of structural SVM (SSVM) classifiers, we apply our idea to the adaptive SSVM (A-SSVM), which only requires the target domain samples together with the existing source-domain classifier for performing the desired adaptation. Altogether, we term our proposal as hierarchical A-SSVM (HA-SSVM). As proof of concept we use HA-SSVM for pedestrian detection and object category recognition. In the former we apply HA-SSVM to the deformable part-based model (DPM) while in the latter HA-SSVM is applied to multi-category classifiers. In both cases, we show how HA-SSVM is effective in increasing the detection/recognition accuracy with respect to adaptation strategies that ignore the structure of the target data. Since, the sub-domains of the target data are not always known a priori, we shown how HA-SSVM can incorporate sub-domain structure discovery for object category recognition.

==> table3.tex <==
\begin{tabular}{|r|r|}\hline 
Method  & Mean\\ \hline 
%SRC (Liblinear) & 38.9 {$\pm$} 0.9\\ \hline 
%SRC (Pegasos) & 39.2 {$\pm$} 0.9\\ \hline 
%SRC (QP-Mosek) & 38.2 {$\pm$} 0.9\\ \hline 
%TAR (Liblinear) & 43.1 {$\pm$} 1.0\\ \hline 
%TAR (Pegasos) & 45.9 {$\pm$} 1.0\\ \hline 
%TAR (QP-Mosek) & 48.8 {$\pm$} 1.1\\ \hline \hline

ASVM & 48.9 {$\pm$} 1.1\\ \hline 
PMT-SVM & 50.0 {$\pm$} 1.1\\ \hline \hline

ARCT     & 49.5 {$\pm$} 0.6          \\ \hline
HFA      & 47.4 {$\pm$} 0.8          \\ \hline
GFK      & 51.0 {$\pm$} 0.7          \\ \hline
MMDT     & 52.9 {$\pm$} 0.9          \\ \hline \hline 

%SRC-SSVM & 42.8 {$\pm$} 0.6\\ \hline 
%TAR-SSVM & 50.3 {$\pm$} 0.9\\ \hline 
%TAR-ALL & 51.9 {$\pm$} 0.7\\ \hline 
ASSVM & 52.9 {$\pm$} 0.7\\ \hline 
TAR-ALL* & \underline{\textit{54.4}} {$\pm$} 0.6\\ \hline 
HASVM & \textbf{56.7} {$\pm$} 0.7\\ \hline 
\end{tabular}


==> table_domainCluster.tex <==
\begin{tabular}{|r|r|r|r|r|}\hline 
  & W D C & A D C & A W C & A W D\\ \hline 

T1 & 34.3 {$\pm$} 1.0 & 34.0 {$\pm$} 1.1 & 32.5 {$\pm$} 1.2 & 32.0 {$\pm$} 1.1\\ \hline 
T2 & 39.1 {$\pm$} 0.6 & 40.4 {$\pm$} 0.5 & 41.5 {$\pm$} 0.7 & 39.3 {$\pm$} 0.6\\ \hline
\end{tabular}

